Compact set-valued deep ensembling in multi-class classification

This paper tackles visible challenges in deep ensemble learning, where deep neural networks serve as ensemble members: training and storage burdens, and robustness of cautious (set-valued) predictions targeting multiple utilities, which may involve reward-sensitivity. To mitigate the training and storage burdens, we propose to employ compact ensembles, such as Bayesian Neural Networks and Convolutional Neural Networks with the Monte-Carlo dropout prediction option, to produce probabilistic predictions. For each query instance, these probabilistic predictions are then used to define a representative distribution optimizing some statistical distance. The representative distribution is then employed to define the Bayes-optimal prediction (BOP) of any utility. To address the potential unrobustness of singleton prediction making, we propose a family of set-utilities satisfying some desirable properties and whose set-valued BOPs can be found efficiently. Empirical evidence is then given to illustrate the potential (dis)advantages of the proposed ensemble learning framework.

==> csv/bnn_cifar10_train_clean_test_clean_mean.tex <==



==> csv/bnn_cifar10_train_clean_test_gnoise_mean.tex <==



==> csv/bnn_cifar10_train_gnoise_test_clean_mean.tex <==



==> csv/bnn_cifar10_train_gnoise_test_gnoise_mean.tex <==



==> csv/bnn_fmnist_train_clean_test_clean_mean.tex <==



==> csv/bnn_fmnist_train_clean_test_gnoise_mean.tex <==



==> csv/bnn_fmnist_train_gnoise_test_clean_mean.tex <==



==> csv/bnn_fmnist_train_gnoise_test_gnoise_mean.tex <==



==> csv/bnn_leaf_train_clean_test_clean_mean.tex <==



==> csv/bnn_leaf_train_clean_test_gnoise_mean.tex <==



==> csv/bnn_leaf_train_gnoise_test_clean_mean.tex <==



==> csv/bnn_leaf_train_gnoise_test_gnoise_mean.tex <==



==> csv/cdo_cifar10_train_clean_test_clean_mean.tex <==



==> csv/cdo_cifar10_train_clean_test_gnoise_mean.tex <==



==> csv/cdo_cifar10_train_gnoise_test_clean_mean.tex <==



==> csv/cdo_cifar10_train_gnoise_test_gnoise_mean.tex <==



==> csv/cdo_fmnist_train_clean_test_clean_mean.tex <==



==> csv/cdo_fmnist_train_clean_test_gnoise_mean.tex <==



==> csv/cdo_fmnist_train_gnoise_test_clean_mean.tex <==



==> csv/cdo_fmnist_train_gnoise_test_gnoise_mean.tex <==



==> csv/cdo_leaf_train_clean_test_clean_mean.tex <==



==> csv/cdo_leaf_train_clean_test_gnoise_mean.tex <==



==> csv/cdo_leaf_train_gnoise_test_clean_mean.tex <==



==> csv/cdo_leaf_train_gnoise_test_gnoise_mean.tex <==



==> csv_nonsense/bnn_cifar10_train_clean_test_clean_mean_nonsense.tex <==



==> csv_nonsense/bnn_cifar10_train_clean_test_gnoise_mean_nonsense.tex <==



==> csv_nonsense/bnn_cifar10_train_gnoise_test_clean_mean_nonsense.tex <==



==> csv_nonsense/bnn_cifar10_train_gnoise_test_gnoise_mean_nonsense.tex <==



==> csv_nonsense/bnn_fmnist_train_clean_test_clean_mean_nonsense.tex <==



==> csv_nonsense/bnn_fmnist_train_clean_test_gnoise_mean_nonsense.tex <==



==> csv_nonsense/bnn_fmnist_train_gnoise_test_clean_mean_nonsense.tex <==



==> csv_nonsense/bnn_fmnist_train_gnoise_test_gnoise_mean_nonsense.tex <==



==> csv_nonsense/bnn_leaf_train_clean_test_clean_mean_nonsense.tex <==



==> csv_nonsense/bnn_leaf_train_clean_test_gnoise_mean_nonsense.tex <==



==> csv_nonsense/bnn_leaf_train_gnoise_test_clean_mean_nonsense.tex <==



==> csv_nonsense/bnn_leaf_train_gnoise_test_gnoise_mean_nonsense.tex <==



==> csv_nonsense/cdo_cifar10_train_clean_test_clean_mean_nonsense.tex <==



==> csv_nonsense/cdo_cifar10_train_clean_test_gnoise_mean_nonsense.tex <==



==> csv_nonsense/cdo_cifar10_train_gnoise_test_clean_mean_nonsense.tex <==



==> csv_nonsense/cdo_cifar10_train_gnoise_test_gnoise_mean_nonsense.tex <==



==> csv_nonsense/cdo_fmnist_train_clean_test_clean_mean_nonsense.tex <==



==> csv_nonsense/cdo_fmnist_train_clean_test_gnoise_mean_nonsense.tex <==



==> csv_nonsense/cdo_fmnist_train_gnoise_test_clean_mean_nonsense.tex <==



==> csv_nonsense/cdo_fmnist_train_gnoise_test_gnoise_mean_nonsense.tex <==



==> csv_nonsense/cdo_leaf_train_clean_test_clean_mean_nonsense.tex <==



==> csv_nonsense/cdo_leaf_train_clean_test_gnoise_mean_nonsense.tex <==



==> csv_nonsense/cdo_leaf_train_gnoise_test_clean_mean_nonsense.tex <==



==> csv_nonsense/cdo_leaf_train_gnoise_test_gnoise_mean_nonsense.tex <==


